Leveraging Code to Improve In-context Learning for Semantic Parsing

In-context learning (ICL) is an appealing approach for semantic parsing due to its few-shot nature and improved generalization. However, learning to parse to rare domain-specific languages (DSLs) from just a few demonstrations is challenging, limiting the performance of even the most capable LLMs. In this work, we improve the effectiveness of ICL for semantic parsing by (1) using general-purpose programming languages such as Python instead of DSLs, and (2) augmenting prompts with a structured domain description that includes, e.g., the available classes and functions. We show that both these changes significantly improve accuracy across three popular datasets. Combined, they lead to dramatic improvements (e.g. 7.9% to 66.5% on SMCalFlow compositional split), nearly closing the performance gap between easier i.i.d.\ and harder compositional splits when used with a strong model, and reducing the need for a large number of demonstrations. We find that the resemblance of the target parse language to general-purpose code is a more important factor than the language's popularity in pre-training corpora. Our findings provide an improved methodology for building semantic parsers in the modern context of ICL with LLMs.

==> todo.tex <==
* Add text describing SQL results [6.2.1]
[Ben] V

* "Indeed, in GeoQuery and Overnight, DD improves performance for DSL on the i.i.d split but to a lesser extent on compositional splits. A possible reason appears to be that DDs primarily help with reducing hallucinations of operators, while using Python helps with improving generalization to unseen structures of programs. Consequently, DSL+DD helps in IID splits but not as much beyond that."
> Add to the results section
[Ben] - on second thought I think it's ok to skip this, as this is just speculation in any case.

limitations/future work:
* "Is the proposed method restricted to semantic parsing, or can it be generalized to other tasks?"
> Add maybe future work to conclusions?

* "My concern is about which conclusions cannot be drawn about the ability of models to generalize compositionally in this setup. In particular, it is not clear to me to what degree the LLM has learned abstract properties of meaning representations/programming languages in general, and to what degree it "peeks" at code from the pre-training data (by varying degrees of memorization). The former should count as compositional generalization, the latter probably not. The fact that the models seem rather brittle to the representation might indicate that the latter might play a role."
Thank you for this clarification! Given our experiment, which shows that even rare PLs can perform well, it seems we can likely rule out at least surface-level memorization. Yet, the actual extent to which LMs generalize versus memorize with respect to the PT corpus remains an important question (pertinent to many of the code generation methods and benchmarks in the field!). We'll make sure to add this point to the limitations section.


> Add something to limitations
[Shivanshu]

* "the related work section presents a very narrow view on methods for compositional generalization and should be expanded. A reader who is not familiar with this area might get the impression that only in-context-learning has been used to achieve compositional generalization when there is work, just to name a few examples, on architectures [1, 2, 3] or data augmentation [4]."
[1] Jonathan Herzig and Jonathan Berant. Span-based semantic parsing for compositional generalization. ACL 2021.
[2] Hao Zheng and Mirella Lapata. Disentangled sequence to sequence learning for compositional generalization. ACL 2022.
[3] Matthias Lindemann, Alexander Koller and Ivan Titov. Compositional Generalization without Trees using Multiset Tagging and Latent Permutations. ACL 2023.
[4] Linlu Qiu, Peter Shaw, Panupong Pasupat, Pawel Nowak, Tal Linzen, Fei Sha, Kristina Toutanova. Improving Compositional Generalization with Latent Structure and Data Augmentation. NACL 2022.
> Add to related work
[Shivanshu]

details:
* what are "discrepancies in the data"?
These include incorrect FunQL annotation or discrepancies in the GeoBase database underlying GeoQuery. An example of the latter is Mount McKinley being called both “Mount McKinley” and just “mckinley” in different places.
> add this example
[Shivanshu]

* Missing details: overnight split, specific version of GPT, table 4 setup
Thank you. We use the split\_0 template split provided in Bogin et al.’s github repository. We used gpt-3.5-turbo-0613. Table 4 refers to the Full DD setup. We will add these details.
> add to experimental setup / appendix
[Ben] V

* We will add depth to our statistics in Table 1.
> Add to table 1
[Ben] V


